Rapidash: Efficient Constraint Discovery via Rapid Verification

Denial Constraint (DC) is a well-established formalism that captures a wide range of integrity constraints commonly encountered, including candidate keys, functional dependencies, and ordering constraints, among others. Given their significance, there has been considerable research interest in achieving fast verification and discovery of exact DCs within the database community. Despite the significant advancements in the field, prior work exhibits notable limitations when confronted with large-scale datasets. The current state-of-the-art exact DC verification algorithm demonstrates a quadratic (worst-case) time complexity relative to the dataset's number of rows. In the context of DC discovery, existing methodologies rely on a two-step algorithm that commences with an expensive data structure-building phase, often requiring hours to complete even for datasets containing only a few million rows. Consequently, users are left without any insights into the DCs that hold on their dataset until this lengthy building phase concludes. In this paper, we introduce Rapidash, a comprehensive framework for DC verification and discovery. Our work makes a dual contribution. First, we establish a connection between orthogonal range search and DC verification. We introduce a novel exact DC verification algorithm that demonstrates near-linear time complexity, representing a theoretical improvement over prior work. Second, we propose an anytime DC discovery algorithm that leverages our novel verification algorithm to gradually provide DCs to users, eliminating the need for the time-intensive building phase observed in prior work. To validate the effectiveness of our algorithms, we conduct extensive evaluations on four large-scale production datasets. Our results reveal that our DC verification algorithm achieves up to 40 times faster performance compared to state-of-the-art approaches.

==> verifast.tex <==
\section{The design of \sys} \label{sec:verification}

In this section, we describe the \sysg algorithm. Our algorithm builds appropriate data structures to store the input data (building phase), leveraging existing work on orthogonal range search and then issues appropriate queries (query phase) to find violations of a given DC. We present various versions of the algorithm depending on whether the two phases are separate or interleaved and discuss the time/space tradeo-ffs. All the variants presented in this work have better complexity that state-of-the-art. {\color{red} Is this correct?}

We first present some background on orthogonal range search that will be useful, before we delve into the details of our algorithm.

\eat{Without loss of generality, we will assume that all predicates of the DC contain only equalities and inequalities but no disequality. \eat{Indeed, any DC containing disequalities can be expanded into a set of equivalent DCs that contain only equalities and inequalities.} We will remove the homogeneous assumption on $\varphi$ later. First, we present some background on orthogonal range search that will be useful.}

\subsection{Orthogonal Range Search}


Given a totally ordered domain $\mathbb{N}$ and let $A$ be a finite subset of $\mathbb{N}^k$ for some $k \geq 1$ of size $N$. Let $\bX = (x_1, \dots, x_k)$ and $\bY = (y_1, \dots, y_k)$ such that $\bX, \bY \in \mathbb{N}^k$ and $x_i \leq y_i$ for all $i \in [k]$. 

\begin{definition}
An orthogonal range search query is denoted by $(\bX, \bY)$, and its evaluation over $A$ consists of enumerating the set 

$$Q(A) = \{ p \in A \mid \bigwedge \limits_{i \in k} x_i \leq p_i \leq y_i \}$$
    
\end{definition}

In other words, $\bX$ and $\bY$ form an axis-aligned hypercube in $k$ dimensions, and $Q(A)$ reports all points in $A$ that lie within the hypercube. The Boolean version of the orthogonal range search problem consists of determining if $Q(A)$ is empty or not. 

\begin{example}
    Consider the tax table $T$ from \autoref{ex:1}. Let $A$ be a set of two-dimensional points obtained from the query $\pi_{\mathtt{Salary}, \mathtt{FedTaxRate}}(\mathtt{Tax})$. Let $\bX = (3500, 17)$ and $\bY = (4500, 22)$. Then, the orthogonal range query $(\bX, \bY)$ is asking for all points such that the \texttt{Salary} is between $3500$ and $4500$, and the \texttt{FedTaxRate} is between $17$ and $22$. In table {\bfseries \texttt{Tax}}, only $t_4$ satisfies the criteria (its values of \texttt{Salary} and \texttt{FedTaxRate} are $4000$ and $10$ respectively). Thus, the result of the orthogonal range search query $(\bX, \bY)$ is $(4000, 10)$. 
\end{example}

Seminal work by Bentley et al.~\cite{bentley1979data} presented two algorithms that can answer orthogonal range search queries efficiently by trading off data structure construction time and space with query answering time. These algorithms leverage two different tree structures (range trees and k-d trees) and their time/space characteristics are presented below.

\begin{theorem}[\cite{bentley1979data}] \label{thm:range}
    Given $N$ k-dimensional points, there exists a data structure, known as a \textbf{range tree}, that can be built in pre-processing time $P(N) = O(N \log^{k-1} N)$, using $S(N) = O(N \log^{k-1} N)$ space, and can answer any orthogonal range search query\footnote{Throughout the paper, we use $\log^k N$ to mean $(\log N)^k$ and not iterated logarithms.} $Q(A)$ in time $T(N) = O(\log^{k-1} N + |Q(A)|)$.
\end{theorem}

\begin{theorem}[\cite{bentley1979data}] \label{thm:kd}
    Given $N$ k-dimensional points, there exists a data structure, known as a \textbf{k-d tree} that can be built in pre-processing time $P(N) = O(N \log N)$, using $S(N) = O(N)$ space, and can answer any orthogonal range search query $Q(A)$ in time $T(N) = O(N^{1-\frac{1}{k}} + |Q(A)|)$.
\end{theorem}

Note that any algorithm that evaluates the orthogonal range search query can solve the Boolean version of the problem by simply stopping the algorithm as soon as we identify that the output is non-empty (i.e. the algorithm is stopped as soon as we know that $|Q(A)| \geq 1$).

Our \sysg algorithm relies on orthogonal range search and can leverage both range and k-d trees. We present experimental results with both variants in Section~\ref{sec:evaluation}. Before presenting the details of the algorithm, we also introduce dynamic range which is used by \sysg for incremental DC verification.

{\color{red} AF: This section needs more work}
\smallskip
\introparagraph{Dynamic range search} Using standard \emph{static-to-dynamic} transformation techniques~\cite{bentley1980decomposable, overmars1983design}, it is well-known that the static data structure for range searching can be transformed into dynamic data structures where the points can be incrementally inserted and deleted. 

\begin{proposition} \label{prop:incremental}
    Given a static range searching data structure with pre-processing time $P(n)$ and query time $T(n)$ on an input of size $n$, there exists a data structure where a point can be inserted in time $O(P(n) \log n / n)$ and the query time is $O(T(n) \log n)$.
\end{proposition}

We note that the data structures generated by the transformation are practical and are shipped in standard programming language libraries~\cite{haskellkd}.





\subsection{Two-phase Verification}

Our basic DC verification algorithm consists of two separate phases (building and querying) and is shown in Algorithm~\ref{algo:main2}. We now briefly describe the algorithm and then provide an example. Without loss of generality, we will focus on homogeneous DCs and assume that all predicates of the DC contain only equalities and inequalities but no disequality. We will remove these assumptions later.

\begin{algorithm}[!t]
	\SetCommentSty{textsf}
	\DontPrintSemicolon 
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\SetKwRepeat{Do}{do}{while}
	\SetKwFunction{rangeSearch}{\textsc{booleanRangeSearch}}
	\SetKwFunction{ins}{\textsc{insert}}
        \SetKwFunction{lowerrange}{\textsc{SearchRange}}
        \SetKwFunction{invertrange}{\textsc{InvertRange}}
	\SetKwProg{myalg}{procedure}{}{}
	\SetKwData{tree}{\textsc{OrthogonalRangeSearchTree}}
	\SetKwData{op}{$\mathsf{op}$}
        \SetKwData{nonEqCount}{$\mathsf{k}$}
	\SetKwData{col}{$\mathsf{col}$}
	\Input{Relation $\R{R}$, Homogeneous DC $\varphi$}
        \Output{True/False}
	\SetKwProg{myproc}{\textsc{procedure}}{}{}
	\SetKwData{ret}{\textbf{return}}
        $\nonEqCount \leftarrow |\vars(\varphi) \setminus \vars_{=}(\varphi)|$ \;
        $H \leftarrow $ empty hash table \;
	\ForEach{$t \in R$}{
            $v \leftarrow \pi_{\vars_{=}(\varphi)} (t)$ \label{line:4}\;
            \If{$v \not\in H$}{
                \If{$\nonEqCount \neq 0$}{
                    $H[v] \leftarrow \text{new } \tree()$ \label{line:5}
                } \Else {
                    $H[v] \leftarrow 1$
                }
            }
            \If{$\nonEqCount \neq 0$}{
                    $\bX, \bY \leftarrow \lowerrange{t}$ \;
                    $\bX', \bY' \leftarrow \invertrange(\bX, \bY)$ \;
            	\If{$H[v].\rangeSearch(\bX, \bY) \lor         
                    H[v].\rangeSearch(\bX', \bY')$ \label{line:search}}{
                        \ret \textbf{false}
                   }
                   $H[v].\ins(\pi_{\vars(\varphi) \setminus \vars_{=}(\varphi)}(t))$
            } \Else {
                $H[v] \leftarrow H[v] + 1$ \label{increment}\;
                \If{$H[v] > 1$}{
                    \ret \textbf{false}
                }
            }
            
        }
        \ret \textbf{true} \;
        \myproc{\lowerrange{t}}{
            $\bX \leftarrow (-\infty, \dots, -\infty), \bY \leftarrow (\infty, \dots, \infty)$ \tcc*{$\bX$ and $\bY$ are indexed by predicate $p_i$. Both are of size $\nonEqCount$}
            \ForEach{predicate $p_i \in \varphi$}{
                \If{$p_i.\op$ is $<$ or $\leq$}{
                    $\bY_i \leftarrow \min \{\bY_i, \pi_{p_i.\col}(t)\}$
                }
                \If{$p_i.\op$ is $>$ or $\geq$}{
                    $\bX_i \leftarrow \max \{\bX_i, \pi_{p_i.\col}(t)\}$
                }
            }
            \ret $\bX, \bY$
        }
        \myproc{\invertrange{$\bX, \bY$}}{
            $\bY' \leftarrow \bX, \bX' \leftarrow \bY$ \;
            flip $-\infty$ to $\infty$ and $\infty$ to $-\infty$ in $\bY'$ and $\bX'$ respectively. \;
            % \ForEach{$i \in \{1, 2, \dots, k\}$}{
            %     \If{$\bY'_i = -\infty $}{
            %         $\bY'_i \leftarrow \infty$
            %     }
            %     \If{$\bX'_i = \infty$}{
            %         $\bX'_i \leftarrow -\infty$
            %     }
            % }
            \ret $\bX', \bY'$
        }
	\caption{{\sc DC verification}}
	\label{algo:main}
\end{algorithm}

\subsection{Interleaved Verification}

Our basic DC verification algorithm consists of two separate phases (building and querying) and is shown in Algorithm~\ref{algo:main2}. However, this distinct two-phase approach does not allow for early termination, i.e., quickly detect violations without requiring to build the entire data structure before hand. 


We now briefly describe the algorithm and then provide an example. Without loss of generality, we will focus on homogeneous DCs and assume that all predicates of the DC contain only equalities and inequalities but no disequality. We will remove these assumptions later.

For each tuple $\tup{t}$ in the input relation, we first project $\tup{t}$ on all columns that participate in an equality predicate. Next, we process the projected tuple based on whether the DC contains only equality predicates or not. If the DC only contains an equality operator in all the predicates, it is sufficient to check if there exist two tuples whose projection over $\vars_{=}(\varphi)$ is equal which would constitute a violation. This is done by storing the count in a hash map which is incremented (line~\ref{increment}). If the DC contains a predicate with inequalities, we build a tree (k-d or range) with the number of dimensions $k$ as the number of columns defined over predicates with inequalities. The $k$ dimensional point inserted into the tree is the tuple obtained by projecting $\tup{t}$ on all non-equality columns. Next, we give an example of how the algorithm works. Figure~\ref{fig:tikz} helps visualizing the ideas behind the example.

\begin{figure}[!htp]
\scalebox{1.1}{
\begin{tikzpicture}
\draw[->,] (0,0)--(5,0);
\draw[->] (0,0)--(0,3.5);
\node[rotate=90] at (-0.6,1.75) {\texttt{FedTaxRate}};
\node[rotate=0] at (2.5, -0.6) {\texttt{Salary}};

\draw (1,0.1) -- (1,-0.1);
\node at (1,-0.2) {$4000$};
\draw (2.5,0.1) -- (2.5,-0.1);
\node at (2.5,-0.2) {$5000$};
\draw (4,0.1) -- (4,-0.1);
\node at (4,-0.2) {$6000$};

\draw (-0.1,1) -- (0.1,1);
\node at (-0.2,1) {$10$};
\draw (-0.1,2) -- (0.1,2);
\node at (-0.2,2) {$15$};
\draw (-0.1,3) -- (0.1,3);
\node at (-0.2,3) {$20$};

\draw[red, fill=red] (1, 3.2) circle[radius=1pt] node[right] {\color{red} $t'_4 = (4000, 22)$};
\draw[fill=black] (1, 1) circle[radius=1pt, fill=black] node[below] {$t_4 = (4000, 10)$};
\draw[fill=black] (2.5, 2) circle[radius=1pt, fill=black] node[below] {$t_2 = (5000, 15)$};
\draw[fill=black] (4, 3) circle[radius=1pt, fill=black] node[below] {$t_3 = (6000, 20)$};


% \draw[->,dotted] (1,1)--(1,3.5);
% \draw[->,dotted] (1,1)--(0.3,1);
% \draw[->,dotted] (1,1)--(5,1);
% \draw[->,dotted] (1,1)--(1,0.2);

\draw[->,dotted] (2.5,2)--(2.5,3.5);
\draw[->,dotted] (2.5,2)--(0.3,2);
\draw[->,dotted] (2.5,2)--(2.5, 0.2);
\draw[->,dotted] (2.5,2)--(5,2);

\draw[fill=gray!80, pattern=north west lines, opacity=0.5] (0,2) -- (2.5,2) -- (2.5,3.5) -- (0,3.5);

\draw[fill=red!80, pattern=north west lines, opacity=0.5, pattern color=blue] (2.5,2) -- (5,2) -- (5, 0) -- (2.5, 0);


% \draw[->,dotted] (4,3)--(4,3.5);
% \draw[->,dotted] (4,3)--(0.3,3);
\end{tikzpicture}}

\caption{\texttt{Salary} and \texttt{FedTaxRate} for each tuple in \texttt{Tax}. The grey (upper left quadrant centered at $t_2$) and blue shaded areas (lower right quadrant centered at $t_2$) show the regions where the tuples that could form a violation $t_2$ lie.}
\label{fig:tikz}
\end{figure}

\begin{example} \label{ex:5}
    Consider the \texttt{Tax} table from our running example and the DC $\varphi_3: (\proj{s}{\mathtt{State}} = \proj{t}{\mathtt{State}} \land \proj{s}{\mathtt{Salary}} \leq  \proj{t}{\mathtt{Salary}} \land \proj{s}{\mathtt{FedTaxRate}} \geq  \proj{t}{\mathtt{FedTaxRate}})$ which contains one equality and two inequality predicates. Algorithm~\ref{algo:main} will first start with the equality predicate, and place $t_1$ in a hash partition by hashing $t_1.\mathtt{State} = \text{New York}$. Since the range tree for the hash bucket is empty, the range search will return false and we insert $(t_1.\mathtt{Salary},$ $t_1.\mathtt{FedTaxRate})$ in the tree. Next, we process $t_2$ which is placed in a different partition since $t_2.\mathtt{State} = \text{Wisconsin}$. The algorithm performs a range search which returns false since the tree corresponding to that partition is empty. We then insert $(5000, 15)$ in the tree. When $t_3$ is processed, it is placed in the same partition as $t_2$ since they have the same $\mathtt{State}$ value. {\color{red} AF: At this point, we have two tuples in the same partition and thus we need to consider the remaining predicates in the DC to establish whether there is a violation. Such a violation would occur in two scenarios: 1) if the tuple already present in the tree ($t_2$) has lower \texttt{Salary} than $6000$ but larger than $20$ \texttt{FedTaxRate} which are the corresponding values of \texttt{Salary} and \texttt{FedTaxRate} for tuple $t_{3}$, or 2) if $t_2$ has salary higher than $6000$ but a \texttt{FedTaxRate} smaller than $20$. To identify whether this is the case, we  perform an orthogonal range search with $\bX = (-\infty, 20)$ and $\bY = (6000, \infty)$ (scenario 1). \eat{In other words, we wish to find if there exists a tuple already present in the tree, such that the first coordinate (i.e. \texttt{Salary}) is smaller than $6000$ but the second coordinate (i.e. \texttt{FedTaxRate}) is larger than $20$. However, it could be the case that there is a tuple in the tree corresponding to a larger salary than $6000$ but a smaller \texttt{FedTaxRate} than $20$.} Then, we also search in the \emph{inverted} range $\bX' = (6000, -\infty)$ and $\bY' = (\infty, 20)$ (scenario 2).} Since there $t_2$ does not lie in in the desired range, both range searches return false and we insert $(6000, 20)$ in the tree. Finally, $t_4$ is processed and placed in the same partition as $t_2$ and $t_3$. We thus query the tree with $\bX = (-\infty, 10)$ and $\bY = (4000, \infty)$ (and the inverted range $\bX' = (4000, -\infty), \bY' = (\infty, 10)$) but no point satisfies the criteria as shown in Figure~\ref{fig:tikz}.

    \smallskip
    \noindent To demonstrate an example of a violation, suppose $t_4.\mathtt{FedTaxRate} = {\color{red} \mathbf{22}}$ (denoted as $t'_4$ in red in Figure~\ref{fig:tikz}). Then, the range search queries would be  $\bX = (-\infty, 22), \bY = (4000, \infty)$ and $\bX' = (4000, -\infty), \bY' = (\infty, 22)$. Then, $t_2$ and $t_3$ form a violation with $t'_4$ since both the points represent a higher salary than $4000$ but a smaller tax rate than $22$.
\end{example}

% \begin{figure}[!htp]
% \scalebox{1.1}{
% \begin{tikzpicture}
% \draw[->,] (0,0)--(5,0);
% \draw[->] (0,0)--(0,3.5);
% \node[rotate=90] at (-0.6,1.75) {\texttt{FedTaxRate}};
% \node[rotate=0] at (2.5, -0.6) {\texttt{Salary}};

% \draw (1,0.1) -- (1,-0.1);
% \node at (1,-0.2) {$4000$};
% \draw (2.5,0.1) -- (2.5,-0.1);
% \node at (2.5,-0.2) {$5000$};
% \draw (4,0.1) -- (4,-0.1);
% \node at (4,-0.2) {$6000$};

% \draw (-0.1,1) -- (0.1,1);
% \node at (-0.2,1) {$10$};
% \draw (-0.1,2) -- (0.1,2);
% \node at (-0.2,2) {$15$};
% \draw (-0.1,3) -- (0.1,3);
% \node at (-0.2,3) {$20$};

% \draw[red, fill=red] (1, 3.2) circle[radius=1pt] node[right] {\color{red} $t'_4 = (4000, 22)$};
% \draw[fill=black] (1, 1) circle[radius=1pt, fill=black] node[below] {$t_4 = (4000, 10)$};
% \draw[fill=black] (2.5, 2) circle[radius=1pt, fill=black] node[below] {$t_2 = (5000, 15)$};
% \draw[fill=black] (4, 3) circle[radius=1pt, fill=black] node[below] {$t_3 = (6000, 20)$};


% \draw[->,dotted] (1,1)--(1,3.5);
% \draw[->,dotted] (1,1)--(0.3,1);
% \draw[->,dotted] (1,1)--(5,1);
% \draw[->,dotted] (1,1)--(1,0.2);

% \draw[->,dotted] (2.5,2)--(2.5,3.5);
% \draw[->,dotted] (2.5,2)--(0.3,2);
% \draw[->,dotted] (2.5,2)--(2.5, 0.2);
% \draw[->,dotted] (2.5,2)--(5,2);

% \draw[fill=gray!80, pattern=north west lines, opacity=0.5] (0,2) -- (2.5,2) -- (2.5,3.5) -- (0,3.5);

% \draw[fill=red!80, pattern=north west lines, opacity=0.5, pattern color=blue] (2.5,2) -- (5,2) -- (5, 0) -- (2.5, 0);


% % \draw[->,dotted] (4,3)--(4,3.5);
% % \draw[->,dotted] (4,3)--(0.3,3);
% \end{tikzpicture}}

% \caption{\texttt{Salary} and \texttt{FedTaxRate} for each tuple in \texttt{Tax}. The grey (upper left quadrant centered at $t_2$) and blue shaded areas (lower right quadrant centered at $t_2$) show the regions where the tuples that could form a violation $t_2$ lie.}
% \label{fig:tikz}
% \end{figure}

We now establish the correctness of Algorithm~\ref{algo:main}.

\begin{lemma}
    Algorithm~\ref{algo:main} correctly determines whether a homogeneous DC $\varphi$ is satisfied.
\end{lemma}
\begin{proof}    We first show that Algorithm~\ref{algo:main} is correct when $\varphi$ only contains equality predicates. In this case, it is sufficient to determine whether there exist two distinct tuples $\tup{s}$ and $\tup{t}$ such that $\pi_{\vars_{=}(\varphi)}(\tup{s}) = \pi_{\vars_{=}(\varphi)}(\tup{t})$. The hash table $H$ stores a counter for each distinct $\pi_{\vars_{=}(\varphi)}(\tup{t})$ and increments it for each tuple $\tup{t} \in R$ (line \ref{increment}). Thus, the algorithm will correctly return false as soon as some counter becomes greater than one and return true only if no such $t_1, t_2$ exists.

Next, we consider the case when there exists at least one predicate with inequality. We show the proof for the case when all inequality predicate operators are $<$, i.e., all predicates in the DC are of the form $(\tup{s}.A = \tup{t}.A)$ or $(\tup{s}.A < \tup{t}.A)$. The proof for other operators is similar. We first state the following claim.

    \begin{claim} \label{claim}
        Let $\vec{v}$ be the set of attributes that appear in the predicates with inequalities. Two tuples $\tup{s}$ and $\tup{t}$ in the same partition can form a violation if and only if $\tup{s}(\vec{v}) \prec \tup{t}(\vec{v})$ or $\tup{t}(\vec{v}) \prec \tup{s}(\vec{v})$\footnote{We use $\tup{s}(\vec{v})$ as a shorthand for $\pi_{\vec{v}}(\tup{s})$}
    \end{claim}
    
    Here, $\prec$ is the standard coordinate-wise strict dominance checking operator. Claim~\ref{claim} follows directly from the operator under consideration and the definition of a violation. Suppose $s$ is the tuple being inserted in the tree. Line~\ref{line:search} will query the range tree with $\bX = (-\infty, \dots, -\infty), \bY = (\pi_{v_1}(\tup{s}), \dots, \pi_{v_k}(\tup{s}))$ and $\bX' = (\pi_{v_1}(\tup{s}), \dots, \pi_{v_k}(\tup{s})),$ $\bY' = (\infty, \dots, \infty)$. In other words, the algorithm searches for a point in the tree such that $\bY$ is strictly smaller or larger for each of the $k$ coordinates. The existence of such a point would imply that there exists some tuple that forms a violation. 
    
    If the orthogonal range search finds no point, then Claim~\ref{claim} tells us that $\tup{s}$ cannot form a violation with any tuple $\tup{t}$ already present in the range tree. In each iteration of the loop, we insert one tuple into the range tree. Therefore, if $t_1$ and $t_2$ form a violation, it will be discovered when one of them (say $t_2$) is already inserted in the range tree and $t_1$ is being processed by the for loop. This completes the proof.
\end{proof}

\introparagraph{Time and Space Complexity} We next establish the running time of the algorithm. First, observe that if $k = 0$, then the algorithm takes $O(|\R{R}|)$ time since the for loop only performs a constant number of hash table operations. If $k \geq 1$, the algorithm performs one insertion and two Boolean orthogonal range search queries in each iteration of the for loop. Assuming the preprocessing time in~\autoref{prop:incremental} can be expressed as $P(n) = n \log^\alpha n$, the running time can be bounded as 

    \begin{align*}
        &\sum \limits_{i = 1}^{|\R{R}|} \Big( \underbrace{\frac{P(i) \cdot \log i}{i}}_{\text{insertion time}} + \underbrace{2 \cdot T(i) \cdot \log i}_{\text{query time}} \Big) \\
        &= \sum \limits_{i = 1}^{|\R{R}|} \Big( \log^{\alpha+1} i +  2 \cdot T(i) \cdot \log i \Big) \\
        &< \int_1^{|\R{R}|+1} \log^{\alpha+1}i\,di + \int_1^{|\R{R}|+1}  2 \cdot T(i) \cdot \log i\,di\\
        &= O(|\R{R}| \cdot \log^{\alpha+1} |\R{R}|) + \int_1^{|\R{R}|}  2 \cdot T(i) \cdot \log i\,di
    \end{align*}

The expressions for insertion and query time come directly from~\autoref{prop:incremental}. The second term in the equation above can be bounded by setting $T(i) = \log^{k-1} i$ or $T(i) = i^{1-1/k}$ if we use \autoref{thm:range} or \autoref{thm:kd} respectively. In both cases, the second term evaluates to $O(|\R{R}| \cdot T(|\R{R}|) \cdot \log |\R{R}|)$. For space usage, note that the hash table takes a linear amount of space in the worst case. Thus, the space requirement of the tree data structure determines the space complexity. The main result can be stated as follows.

\begin{theorem} \label{thm:main}
    Let $P(n) = n \log^{\alpha} n$ denote the construction time, $S(n)$ the space requirement, and $T(n)$ denote the query time of a static orthogonal range search data structure consisting of $n$ points. Then, Algorithm~\ref{algo:main} runs in time $O(|\R{R}| \cdot \log|\R{R}| \cdot (\log^\alpha|\R{R}| + T(|\R{R}|)))$ and uses space $S(|\R{R}|)$.
\end{theorem}

\begin{algorithm}[!t]
	\SetCommentSty{textsf}
	\DontPrintSemicolon 
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\SetKwRepeat{Do}{do}{while}
	\SetKwFunction{rangeSearch}{\textsc{booleanRangeSearch}}
	\SetKwFunction{ins}{\textsc{insert}}
        \SetKwFunction{lowerrange}{\textsc{SearchRange}}
        \SetKwFunction{invertrange}{\textsc{InvertRange}}
        \SetKwFunction{len}{\textsc{len}}
	\SetKwProg{myalg}{procedure}{}{}
	\SetKwData{tree}{\textsc{OrthogonalRangeSearchTree}}
	\SetKwData{op}{$\mathsf{op}$}
        \SetKwData{nonEqCount}{$\mathsf{k}$}
	\SetKwData{col}{$\mathsf{col}$}
	\Input{Relation $\R{R}$, Homogeneous DC $\varphi$}
        \Output{True/False}
	\SetKwProg{myproc}{\textsc{procedure}}{}{}
	\SetKwData{ret}{\textbf{return}}
        $\nonEqCount \leftarrow |\vars(\varphi) \setminus \vars_{=}(\varphi)|$ \;
        $H,T \leftarrow $ empty hash table \;
	\ForEach{$t \in R$ \label{line:for}}{
            $v \leftarrow \pi_{\vars_{=}(\varphi)} (t)$ \label{line:4}\;
            \If{$v \not\in H$}{
                $H[v] \leftarrow $ new List()
            }
            $H[v].\ins(\pi_{\vars(\varphi) \setminus \vars_{=}(\varphi)}(t))$ \;
            \If{$\nonEqCount = 0 \land H[v].\len() > 1$}{
                \ret \textbf{false}        
            }
        }
        \ForEach{bucket $b \in H$}{
            $T[b] \leftarrow $ create \tree\ for all points in $H[b]$ \label{line:build}\;
            \ForEach{$t \in H[b]$}{
                $\bX, \bY \leftarrow \lowerrange{t}$ \tcc*{From Algorithm~\ref{algo:main}}
                %$\bX', \bY' \leftarrow \invertrange(\bX, \bY)$ \;
                \If{$T[b].\rangeSearch(\bX, \bY)$ \label{line:query}}{
                        \ret \textbf{false}
                }
            }
            free space used by $T[b]$
        }
        \ret \textbf{true}
	\caption{{\sc Batched DC verification}}
	\label{algo:main2}
\end{algorithm}



\subsection{Batched Verification} \autoref{thm:main} contains logarithmic factors that can be optimized further. Algorithm~\ref{algo:main2} shows the batched version that constructs the data structure first before querying. The algorithm begins similarly to Algorithm~\ref{algo:main} where we partition the input into hash buckets by using the projection on equality predicates as the key. The key difference is that instead of building the tree and querying \emph{on-the-fly} in each iteration, we first build the tree for all tuples (line~\ref{line:build}), and then query it in a separate loop (line~\ref{line:query}). This separation allows us to avoid the logarithmic factors that come from the static-to-dynamic transformation. The correctness of~\autoref{algo:main2} readily follows from \autoref{thm:main}. The running time can be bounded similarly to \autoref{thm:main} by observing that the for loop on \autoref{line:for} takes time $O(|\R{R}|)$, range tree construction takes time $P(|\R{R}|)$ and we perform one range query for each tuple in the input. Thus, the total time taken is $P(|\R{R}|) + \sum \limits_{i=1}^{|\R{R}|} T(|\R{R}|)$. Since we free up space after processing each partition, the space requirement is dominated by the partition that contains the largest number of tuples.

\begin{theorem} \label{thm:main2}
    Let $P(n) = n \log^{\alpha} n$ denote the construction time, $S(n)$ the space requirement, and $T(n)$ denote the query time of a static orthogonal range search data structure consisting of $n$ points. Then, Algorithm~\ref{algo:main2} runs in time $O(|\R{R}| \cdot (\log^\alpha|\R{R}| + T(|\R{R}|)))$ and uses space $S(|\R{R}|)$.
\end{theorem}

\eat{\smallskip
\introparagraph{Improving Batched DC verification} Algorithm~\ref{algo:main2} can be further optimized by shaving off another log factor from the running time. The key idea is that we can sort the relation $\R{R}$ on one of the columns (say $C^\star$) that participates in a predicate with inequality. The comparator function used for sorting is $\op$ in the predicate. For $<$ and $>$ operators, we also keep track of whether there is at least one tuple pair that satisfies the predicate by keeping track of the minimum and maximum value of column $C^\star$.

When creating the range tree, we can now ignore column $C^\star$, thus reducing the dimensions of the points inserted in the range tree by one. \TODO{add statement and proof?}}

\begin{algorithm}[!t]
	\SetCommentSty{textsf}
	\DontPrintSemicolon 
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\SetKwRepeat{Do}{do}{while}
	\SetKwFunction{rangeSearch}{\textsc{booleanRangeSearch}}
	\SetKwFunction{ins}{\textsc{insert}}
        \SetKwFunction{lowerrange}{\textsc{SearchRange}}
        \SetKwFunction{invertrange}{\textsc{InvertRange}}
        \SetKwFunction{len}{\textsc{len}}
	\SetKwProg{myalg}{procedure}{}{}
	\SetKwData{tree}{\textsc{OrthogonalRangeSearchTree}}
	\SetKwData{op}{$\mathsf{op}$}
        \SetKwData{nonEqCount}{$\mathsf{k}$}
	\SetKwData{col}{$\mathsf{col}$}
	\Input{Relation $\R{R}$, Homogeneous DC $\varphi$}
        \Output{True/False}
	\SetKwProg{myproc}{\textsc{procedure}}{}{}
	\SetKwData{ret}{\textbf{return}}
        $\nonEqCount \leftarrow |\vars(\varphi) \setminus \vars_{=}(\varphi)|$ \;
        $H,T \leftarrow $ empty hash table \;
	\ForEach{$t \in R$ \label{line:for}}{
            $v \leftarrow \pi_{\vars_{=}(\varphi)} (t)$ \label{line:4}\;
            \If{$v \not\in H$}{
                $H[v] \leftarrow $ new List()
            }
            $H[v].\ins(\pi_{\vars(\varphi) \setminus \vars_{=}(\varphi)}(t))$ \;
            \If{$\nonEqCount = 0 \land H[v].\len() > 1$}{
                \ret \textbf{false}        
            }
        }
        \ForEach{bucket $b \in H$}{
            $T[b] \leftarrow $ create \tree\ for all points in $H[b]$ \label{line:build}\;
            \ForEach{$t \in H[b]$}{
                $\bX, \bY \leftarrow \lowerrange{t}$ \tcc*{From Algorithm~\ref{algo:main}}
                %$\bX', \bY' \leftarrow \invertrange(\bX, \bY)$ \;
                \If{$T[b].\rangeSearch(\bX, \bY)$ \label{line:query}}{
                        \ret \textbf{false}
                }
            }
            free space used by $T[b]$
        }
        \ret \textbf{true}
	\caption{{\sc Batched DC verification}}
	\label{algo:main2}
\end{algorithm}

\smallskip
\introparagraph{Discussion} Although the running time guarantees of \autoref{thm:main} and \autoref{thm:main2} only differ by a logarithmic factor in the worst-case, the performance on specific relations can vary significantly as shown below.

\begin{proposition}
    For every homogeneous DC $\varphi$ with at least one inequality predicate, there exists a relation $\R{R}$ such that Algorithm~\ref{algo:main} takes $O(1)$ time and Algorithm~\ref{algo:main2} requires $\Omega(|\R{R}|)$ time.
\end{proposition}
\begin{proof}
    We sketch the proof for $\varphi : \forall \tup{s}, \tup{t} \in \R{R},\ \neg (\tup{s}.A < \tup{t}.A)$ which can be extended straightforwardly for other DCs of interest. We construct a unary relation $\R{R}(A)$ of size $N$ as follows: the first tuple $t_1$ is $1$ and the remaining $N-1$ tuples are $2$. Note that $t_1$ forms a violation with every other tuple in the relation. Algorithm~\ref{algo:main} initializes one range tree for all the tuples since there is no equality predicate. After $t_1$ has been inserted, and the next tuple $t_2$ is inserted, the range search query will return true and the algorithm will terminate. Note that all the operations take $O(1)$ time since the tree only contains two tuples. However, Algorithm~\ref{algo:main2} requires $\Omega(|\R{R}|)$ time for the partitioning of the input in the for loop on~\autoref{line:for}.
\end{proof}

\smallskip
\noindent In other words, the lemma above says that \autoref{thm:main} has the advantage of terminating early and returning an answer since it builds the range tree incrementally and does the querying of the data structure on-the-fly. On the other hand, \autoref{algo:main2} requires $\Omega(|\R{R}|)$ of processing before it can start querying the range trees. When using k-d trees, \autoref{algo:main2} also has the advantage of using a straightforward construction~\cite{brown2015building} as opposed to using the static-to-dynamic transformation which is more involved in terms of creating multiple trees~\cite{overmars1983design}.

\smallskip
\introparagraph{Improved Processing for certain predicates} The processing of all homogeneous predicates of the form $\proj{s}{\A{A}}\ \op\ \proj{s}{\A{A'}}$ can be done straightforwardly as follows. For each $\tup{s} \in \R{R}$, we can evaluate each predicate in constant time since we only need to look at one tuple at a time. If any of the predicates evaluates to false, we can remove $\tup{t}$ from consideration since it will form a violation with every  tuple. As an example, for the \texttt{Tax} table, suppose we have the DC $\neg (\proj{s}{\mathtt{Salary}} \leq \proj{s}{\mathtt{FedTaxRate}})$, i.e., we wish to verify whether the \texttt{Salary} is strictly larger than the  \texttt{FedTaxRate}. Checking this condition can be done as the first step in the top-level loop of the algorithms we have seen so far.

\subsection{Heterogeneous DC}

DCs containing predicates of the form $\proj{s}{\A{A}}\ \op \ \proj{t}{\A{A'}}$ can also be processed using range search queries but requires a different range query building technique. For each such predicate, we insert $\proj{s}{\A{A}}$ as a dimension (say $\ell^{th}$ dimension) in the range tree. However, when creating the vectors $\bX, \bY$, we use $\proj{t}{\A{A'}}$ as the value at position $\ell$ in the vectors. We illustrate with the help of an example.

\begin{example}
    Consider the DC $\varphi: \neg (\proj{s}{\mathtt{Salary}}\ \leq \ \proj{t}{\mathtt{FedTaxRate}})$. This constraint says that \texttt{Salary} must be strictly larger than \emph{all} values that \texttt{FedTaxRate} takes in the \texttt{Tax} table. Suppose we are processing tuple $r \in 
    \R{R}$. When constructing the tree structure, we insert the one-dimensional point $\proj{r}{\mathtt{Salary}}$. For \texttt{Tax}, after $t_1.\mathtt{Salary} = 3000$ has been inserted and $t_2$ is being processed, the range query will be $\bX = (-\infty), \bY = (15)$. In words, this range query corresponds to finding a point in the tree that has a value smaller than $15$. Since we are inserting \texttt{Salary} into the tree, if the range query finds a point smaller than $15$, it would correspond to a tuple that has \texttt{Salary} smaller than $15$, thus discovering a violation.
\end{example}

\subsection{Other Optimizations} \label{subsec:opt}

In this section, we discuss optimizations that improve the running time for verifying DCs with special structures.

\smallskip
\introparagraph{Disequality predicate} We begin by first removing the assumption about the DC containing no disequality operators. First, any predicate $\proj{s}{\A{A}}\ \neq\ \proj{t}{\A{B}}$ can be written as a union of two predicates: $(\proj{s}{\A{A}}\ <\ \proj{t}{\A{B}}) \lor (\proj{s}{\A{A}}\ >\ \proj{t}{\A{B}})$. Therefore, a DC containing $\ell$ predicates with $\op$ as $\neq$ can be equivalently written as a conjunction of $2^{\ell}$ DCs containing no disequality operator.

If the original DC contains no inequality predicate, then it is possible to reduce the number of equivalent DCs from $2^{\ell}$ to $2^{\ell-1}$. The idea is that a violation $(\tup{s}, \tup{t})$ is symmetric (i.e. $(\tup{t}, \tup{s})$ is also a violation) if the DC contains only equality and disequality predicates. Therefore, when converting a DC to only have inequalities, it suffices to expand $(\tup{s}.A \ \neq \ \tup{t}.A)$ to just $(\tup{s}.A \ < \ \tup{t}.A)$ for one the last disequality predicate instead of $(\tup{s}.A \ < \ \tup{t}.A) \lor (\tup{s}.A \ > \ \tup{t}.A)$. The same observation also applies when the predicate is heterogeneous.

\begin{proposition}
    Given a DC $\varphi$ with only equality and $\ell$ disequality predicates, there exists a conjunction of $2^{\ell-1}$ DCs that contain only equality and inequality predicates.
\end{proposition}
\begin{proof}
    We sketch the proof for a homogenous DC. Consider a violation $(\tup{s}, \tup{t})$ for $\varphi$. Without loss of generality, suppose $\tup{s} \prec \tup{t}$ on the $\ell$ coordinates.
    Since $(\tup{t}, \tup{s})$ is also a violation, \TODO{finish this}
\end{proof}


\smallskip
\introparagraph{Inequality predicate} If a DC has at most one predicate (homogeneous or heterogeneous) containing an inequality, then the verification can be done in linear time. Algorithm~\ref{algo:het} shows the main steps when the inequality predicate is heterogeneous. The algorithm for homogeneous inequality predicate is very similar. Like the previous algorithms, we begin by partitioning the input into a hash table based on the equality predicates. Lines~\ref{line:min}-\ref{line:max} store the min and max values for every column in the table. The key insight is that for a violation formed by $s, t$ it must hold that $\proj{s}{\A{A}} \op \ \proj{t}{\A{A'}}$ is true. Let us fix $\op$ to $<$. Then, $\proj{t}{\A{A'}}$ must be less than or equal to the smallest value in column $A$ to form a violation. This is precisely the condition checked on line~\ref{line:if}. The algorithm makes only three passes for the entire dataset and the overall time complexity is $O(|\R{R}|)$. While this optimization is simple, it has important implications. In particular, popular constraints such as functional dependencies (FD) are DCs that contain exactly one inequality predicate. Algorithm~\ref{algo:het} recovers the linear time algorithm to verify FDs~\cite{ibaraki1999functional} and candidate keys. However, it is not clear that prior work can achieve the same provable guarantee.

\begin{table*}[!htp]
\caption{Summary of the main results} \label{table:summary}
\scalebox{1.0}{
 \begin{tabularx}{\linewidth}{ l  @{\extracolsep{\fill}} l l l} 
 \toprule
 Algorithm & Answering time & Space & Comments \\
 \midrule
Algorithm~\ref{algo:main} with range tree & $O(|\R{R}| \log^k |\R{R}|)$ & $O(|\R{R}| \log^{k-1} |\R{R}|)$  &  early termination\\

Algorithm~\ref{algo:main} with k-d tree & $O(|\R{R}|^{2-\frac{1}{k}} \log |\R{R}|)$ & $O(|\R{R}|)$ & early termination \\
\midrule
Algorithm~\ref{algo:main2} with range tree & $O(|\R{R}| \log^{k-1}|\R{R}|)$ & $O(|\R{R}| \log^{k-1} |\R{R}|)$  & batched version;  no early termination \\

Algorithm~\ref{algo:main2} with k-d tree & $O(|\R{R}|^{2-\frac{1}{k}})$ & $O(|\R{R}|)$  & batched version;  no early termination \\
\midrule
Algorithm~\ref{algo:main3} with range tree & $O(|\R{R}| (\log^{k-1}|\R{R}| + \log |\R{R}|))$ & $O(|\R{R}| \log^{k-1} |\R{R}|)$  & hybrid;  requires sorting \\

Algorithm~\ref{algo:main3} with k-d tree & $O(|\R{R}|^{2-\frac{1}{k-1}} \log |\R{R}|)$ & $O(|\R{R}|)$  & hybrid; $k \geq 2$;  requires sorting \\
\bottomrule
 \end{tabularx}
 }
 \end{table*}

\begin{algorithm}[!t]
	\SetCommentSty{textsf}
	\DontPrintSemicolon 
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\SetKwRepeat{Do}{do}{while}
	\SetKwFunction{rangeSearch}{\textsc{booleanRangeSearch}}
	\SetKwFunction{ins}{\textsc{insert}}
        \SetKwFunction{lowerrange}{\textsc{SearchRange}}
	\SetKwProg{myalg}{procedure}{}{}
	\SetKwData{tree}{\textsc{OrthogonalRangeSearchTree}}
	\SetKwData{op}{$\mathsf{op}$}
        \SetKwData{nonEqCount}{$\mathsf{k}$}
        \SetKwData{min}{$\mathsf{min}$}
        \SetKwData{max}{$\mathsf{max}$}
        \SetKwFunction{List}{\textsc{list}}
        \SetKwFunction{last}{\textsc{last}}
        \SetKwFunction{first}{\textsc{first}}
	\SetKwData{col}{$\mathsf{col}$}
	\Input{Relation $\R{R}$, DC $\varphi$ with some equality and one heterogeneous inequality predicate $p$}
        \Output{True/False}
	\SetKwProg{myproc}{\textsc{procedure}}{}{}
	\SetKwData{ret}{\textbf{return}}
        \SetKwData{flag}{isViolation}
        $H \leftarrow $ empty hash table \;
	\ForEach{$t \in R$}{
            $v \leftarrow \pi_{\vars_{=}(\varphi)} (t)$ \label{line:4}\;
            \If{$v \not\in H$}{
                    $H[v] \leftarrow \text{new } \List()$
            }
            $H[v].\ins(t)$ \\
            \tcc{Let $b$ be the bucket to which $t$ is hashed}
            \For{$v \in \{A, A'\}$}{
                    $\min^b_v \leftarrow \min \{\min^b_v, t[v]\}$ \; \label{line:min}
                    $\max^b_v \leftarrow \max \{\max^b_v, t[v]\}$ \; \label{line:max}
            }
            \If{$(p.\op \in \{<, \leq\} \land \neg (\min^b_{A} \ \op \ t.A')) \lor (p.\op \in \{>, \geq\} \land \neg (\max^b_{A} \ \op \ t.A'))$ \label{line:if}}{
                    \ret \textbf{false}
                }
        }
        % \ForEach{bucket $b \in H$}{
        %     \ForEach{$t \in H[b]$}{
                
        %     }
        % }
        \ret \textbf{true} \;
	\caption{{\sc DC verification for Heterogeneous predicate}}
	\label{algo:het}
\end{algorithm}


\subsection{Hybrid Verification}

We next present an interesting variant that combines the properties of the two algorithms that we have seen so far. The key idea is that we can sort the relation $\R{R}$ on one of the columns (say $C^\star$) that participates in a predicate with the inequality $<$ or $>$\footnote{The technique also works with $\leq$ and $\geq$ but requires a more involved construction which we omit due to space constraints.}. The comparator function used for sorting is $\op$ in the predicate. When creating the range tree, we can now ignore column $C^\star$, thus reducing the dimensions of the points inserted in the range tree by one. We demonstrate with the help of an example.

\begin{algorithm}[!t]
	\SetCommentSty{textsf}
	\DontPrintSemicolon 
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\SetKwRepeat{Do}{do}{while}
	\SetKwFunction{rangeSearch}{\textsc{booleanRangeSearch}}
	\SetKwFunction{ins}{\textsc{insert}}
        \SetKwFunction{lowerrange}{\textsc{SearchRange}}
        \SetKwFunction{append}{\textsc{append}}
        \SetKwFunction{invertrange}{\textsc{InvertRange}}
        \SetKwFunction{len}{\textsc{len}}
	\SetKwProg{myalg}{procedure}{}{}
	\SetKwData{tree}{\textsc{OrthogonalRangeSearchTree}}
        \SetKwData{partition}{\textsc{HashPartition}}
	\SetKwData{op}{$\mathsf{op}$}
        \SetKwData{st}{$\mathsf{start}$}
        \SetKwData{ed}{$\mathsf{end}$}
        \SetKwData{nonEqCount}{$\mathsf{k}$}
	\SetKwData{col}{$\mathsf{col}$}
	\Input{Relation $\R{R}$, Homogeneous DC $\varphi$}
        \Output{True/False}
	\SetKwProg{myproc}{\textsc{procedure}}{}{}
	\SetKwData{ret}{\textbf{return}}
 \tcc{$C^\star$ participates in a predicate $p$ with $\op \in \{<,>\}$}
        $H \leftarrow \partition{\R{R}}$ \tcc{partition on $\vars_{=}(\varphi)$}
         $T \leftarrow $empty hash table \;
        \ForEach{bucket $b \in H$}{
            $\R{R}_b \leftarrow $ sorted list all tuples in $H[b]$ on column $C^\star$ \;
            $\mL \leftarrow \emptyset$ \;
            $T[b] \leftarrow \tree{}$ \;
            \For{$i \in \{0, \dots |\R{R}_b|-1\}$}{
                $\bX, \bY \leftarrow \lowerrange(t_i)$ \tcc*{From Algorithm~\ref{algo:main}}
                %$\bX', \bY' \leftarrow \invertrange(\bX, \bY)$ \;
                \If{$T[b].\rangeSearch(\bX, \bY)$}{
                        \ret \textbf{false}
                }
                \If{$t_i.C^\star < t_{i+1}.C^\star$}{
                    \If{$\mL \neq \emptyset$}{
                        \ForEach{$s \in \mL$}{
                            $H[v].\ins(\pi_{\vars(\varphi) \setminus \{\vars_{=}(\varphi),C^\star\}}(s))$
                        }
                        $\mL \leftarrow \emptyset$
                    } \Else{
                        $H[v].\ins(\pi_{\vars(\varphi) \setminus \{\vars_{=}(\varphi),C^\star\}}(t_i))$
                    }
                } \Else{
                    $\mL.\append{t_i}$
                }
            }
        }
        \ret \textbf{true}
	\caption{{\sc Hybrid DC verification}}
	\label{algo:main3}
\end{algorithm}

\begin{example}
    Let us look at the processing of $\psi: (\proj{s}{\mathtt{State}} = \proj{t}{\mathtt{State}} \land \proj{s}{\mathtt{Salary}} <  \proj{t}{\mathtt{Salary}} \land \proj{s}{\mathtt{FedTaxRate}} \geq  \proj{t}{\mathtt{FedTaxRate}})$ using range trees. First, we sort \texttt{Tax} on \texttt{Salary} in ascending order and then remove the column. This step orders the tuples as $t_1, t_4, t_2, t_3$. This order guarantees that when we process a tuple $s$, it can form a violation only with tuples that appear before $s$. When $t_4$ is processed, the 1D tree is empty (note that $t_1$ belongs to a different partition). When $t_2$ is processed, the tree contains point $10$ (which is $t_4.\mathtt{FedTaxRate}$) and $t_2.\mathtt{FedTaxRate} = 15$ is larger than $10$. Since we are looking for a point that has a value of at least $10$ and there is none in the tree, we continue processing. However, if $t_4.\mathtt{FedTaxRate} = {\color{red} 22}$, then $t_2$ would form a violation with $t_2$ since $t_4$ has a higher salary but lower tax rate. Thus, the worst-case processing time for $\varphi_3$ will only be $O(|\R{R}| \log |\R{R}|)$ instead of $O(|\R{R}| \log^2 |\R{R}|)$.
\end{example}

Algorithm~\ref{algo:main3} has the desirable property of avoiding building the tree structure completely before we begin querying. Instead it only requires sorting the dataset, which is cheaper. In many cases, the dataset may already be sorted on some column that is used in a DC predicate, thus avoiding the need to sort altogether. We conclude the section by summarizing the main results obtained from this section in~\autoref{table:summary}.

